Data Leakage via Access Patterns of Sparse Features in Deep Learning-based Recommendation Systems

Online personalized recommendation services are generally hosted in the cloud where users query the cloud-based model to receive recommended input such as merchandise of interest or news feed. State-of-the-art recommendation models rely on sparse and dense features to represent users' profile information and the items they interact with. Although sparse features account for 99% of the total model size, there was not enough attention paid to the potential information leakage through sparse features. These sparse features are employed to track users' behavior, e.g., their click history, object interactions, etc., potentially carrying each user's private information. Sparse features are represented as learned embedding vectors that are stored in large tables, and personalized recommendation is performed by using a specific user's sparse feature to index through the tables. Even with recently-proposed methods that hides the computation happening in the cloud, an attacker in the cloud may be able to still track the access patterns to the embedding tables. This paper explores the private information that may be learned by tracking a recommendation model's sparse feature access patterns. We first characterize the types of attacks that can be carried out on sparse features in recommendation models in an untrusted cloud, followed by a demonstration of how each of these attacks leads to extracting users' private information or tracking users by their behavior over time.

==> 10.Experiments.tex <==
\section{Experiments}
\label{sec:exp}
\subsection{Datasets}


\textbf{Kaggle Display Advertising dataset}

\textbf{Criteo Terabyte Dataset}


\textbf{Taobao User Behaviour}: \urlhttps{https://tianchi.aliyun.com/dataset/dataDetail?dataId=649&userId=1}

Dataset is randomly selected from 1 million users who have behaviors including click, purchase, adding item to shopping cart and item favoring during November 25 to December 03, 2017. The dataset is organized in a very similar form to MovieLens-20M, i.e., each line represents a specific user-item interaction, which consists of user ID, item ID, item's category ID, behavior type and timestamp, separated by commas; e.g (uid, iid, cid, ctag, time). 


* Uid = An integer, the serialized ID that represents a user
* iid = An integer, the serialized ID that represents an item
* cid = A string, enum-type from ('pv', 'buy', 'cart', 'fav'):
    * pv: Page view of an item's detail page, equivalent to an item click
    * buy: Purchase an item
    * cart: Add an item to shopping cart
    * fav: Favor an item
time = An integer, the timestamp of the behavior
* Dataset Characteristics:
* Number of Users = 987,994
* Number of Items = 4,162,024
* Number of Categories = 9,439
* Number of Interactions = 100,150,807

\textbf{Taobao Ads Display}
This dataset consists of four different raw data files. User profile data file stores static user features including user id (1.14M), micro group id (97), group id (13), gender (2), age level (7), consumption grade/plevel (4), shopping depth (3), occupation/is college student (2), city level (5). User Behavior file contains dynamic user history behaviour such as user id (1.14M), btag (4: brows, cart, favor, buy), category id (13K), brand(100 K), and timestamp (dense). This file contains 723268134 interaction histories. 

Item Features:
ad id (847K), category id (13(11)K), campaign id (423K), advertiser id (256K), brand id (100(304)K), price (dense)

Raw Sample:
Randomly sampled 1.14 users over 8 days.
User id (1.14M), ad id (847K), nonclk, clk, timestamp

\begin{itemize}
    \item Accuracy analysis for Hash inversion attack
    \item Accuracy analysis for frequnecy-based attack and the effect of observed queries and different pre-hash distribution on the accuracy
    \item Execution time analysis of frequency based attack Vs number of observed samples Vs accuracy
    \item Accuracy analysis of re-identification attack 
\end{itemize}

\begin{comment}
\subsection{Comparison}
\begin{itemize}
    \item PathORAM/Recursive PathORAM implemented in SGX
    \item Pancake with replica map protection in SGX
    \item performance as a function of block size in PathOram parts
    \item Combining clustering with both of the ideas
    \item Time per query comparison between solutions and with different number of entries and dimension in the embedding table
    \item Memory consumption comparison between solutions
    \item accuracy degradation Vs memory/latency utliziation in clustering
    \item other ORAM investigations!
\end{itemize}
\end{comment}
\subsection{Effect of Clustering in Accuracy of Different Attacks}

==> 4.Attack.tex <==
\section{Attacks Against Recommendation Systems}
\label{sec:attacks}
\begin{comment}
\begin{table*}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{\textbf{Type of Information}} & {\begin{tabular}[c]{@{}l@{}}\textbf{Dense Features}\\ \textbf{(User Inputs)}} \end{tabular}&{\begin{tabular}[c]{@{}l@{}}\textbf{Sparse Features}\\ \textbf{(User Inputs)}} \end{tabular}& {\textbf{Labels}} & {\begin{tabular}[c]{@{}l@{}}\textbf{Hidden FeatureMaps}\\ \textbf{(Intermedi
ate values)}} \end{tabular}& {\begin{tabular}[c]{@{}l@{}}\textbf{Model Update}\\ \textbf{Values}} \end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Model Parameters} \\ \textbf{(Embedding Table Values}\\\textbf{MLP Parameters)}\end{tabular} \\ \hline
& Identification &   \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{red}{\xmark}   & \textcolor{blue}{\cmark}&   \textcolor{blue}{\cmark} &  \textcolor{blue}{\cmark} \\ \cline{2-8} 

& {Re-identification} &\textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{red}{\xmark}   & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark} &  \textcolor{blue}{\cmark} \\ \cline{2-8} 
& Sensitive Information & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{red}{\xmark}   & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark} &  \textcolor{blue}{\cmark} \\ \cline{2-8} & Membership Inference &\textcolor{red}{\xmark} &   \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}   & \textcolor{red}{\xmark}&   \textcolor{red}{\xmark} &  \textcolor{blue}{\cmark} \\ \cline{2-8}& Model Inversion &\textcolor{red}{\xmark} &   \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}  & \textcolor{red}{\xmark} &   \textcolor{red}{\xmark} &  \textcolor{blue}{\cmark} \\ \cline{2-8} 
\multirow{-7}{*}{\begin{tabular}[c]{@{}l@{}}Attack\\ Type\end{tabular}} & Model stealing &\textcolor{red}{\xmark} &   \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}   & \textcolor{red}{\xmark} &   \textcolor{red}{\xmark} &  \textcolor{blue}{\cmark}            \\ \hline
& User Feature Values   &     \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{blue}{\cmark}   & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark} &  \textcolor{blue}{\cmark}   \\ \cline{2-8}      & User Feature Distribution                         &     \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{blue}{\cmark}   & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark} &  \textcolor{blue}{\cmark}                                                                              \\ \cline{2-8} 
\multirow{-3}{*}{Information}                                           & Company IP    &   \textcolor{red}{\xmark} &   \textcolor{red}{\xmark}  & \textcolor{red}{\xmark}   & \textcolor{red}{\xmark}&   \textcolor{red}{\xmark} &  \textcolor{red}{\xmark}    \\ \hline
 & Training       &   \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{blue}{\cmark}   & \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}&  \textcolor{blue}{\cmark}                                                                      \\ \cline{2-8} 
\multirow{-2}{*}{Phase}                                                 & Inference  &   \textcolor{blue}{\cmark} &   \textcolor{blue}{\cmark}  & \textcolor{red}{\xmark}   & \textcolor{blue}{\cmark} &   \textcolor{red}{\xmark} &  \textcolor{blue}{\cmark}                                                                                                           \\ \hline
\end{tabular}
}
\end{table*}
\end{comment}
 %This information is sensitive in health-care applications when the same user sends multiple queries. This attack plays an important role when the attacker have access to multiple systems and can Re-Identify the same user within multiple systems. %feedback needed

%\textbf{Distribution Leak (NOT SURE IF WE WANT TO INCLUDE THIS).} Even if the attacker cannot find out the feature values of the users, changes in the distribution can be observed over time. In some applications, such as political applications this information is sensitive because it can indicate a shift in people's opinions.

\begin{comment}
\textbf{Membership Inference.} Given a data instance and (black-box or white-box) access to a pre-trained target model, a membership inference attack speculates whether or not the given data instance has contributed to the training step of the target model~\cite{zhang2021membership}. 
One difference between the Machine Learning Membership attack~\cite{zhang2021membership} and this attack in recommendation systems is that the output in recommendation systems is that the adversary can only observe the ordered recommended items from a recommendation system instead of prediction results in the form of posterior probabilities.

\textbf{Model Inversion.} The model inversion attack extracts information from the training data used for learning the model. For a given class, the attacker, with either black-box or white-box access to the model, attempts to create an input that maximizes the confidence score of that class using the gradient descent algorithm.

\textbf{Model Stealing.} Trained models are considered the intellectual properties of their owners and can be considered confidential in many cases, therefore, extracting the model is considered a privacy breach. Apart from this, DNNs are shown to memorize information about their training data, therefore exposing the model parameters could lead to model inversion attack. A model stealing attack is meant to recover the model parameters via black-box access to the target model.
\end{comment}
\begin{comment}
\textbf{Identification attack (Direct information exposure)}. There is the direct risk that someone will learn information that the user wishes to keep private. For example, revealing identifiable information could lead to identity theft. One example is the social security number. Also, a combination of attributes may become highly identifiable. Such a combination is called a quasi-identifier to differentiate them from directly identifiable info such as social security numbers. The combination of 5-digit zip code, birthdate, and gender is considered a quasi-identifier as shown in~\cite{lam2006you}.

\textbf{Sensitive attribute inference attacks.} In this attack, the adversary’s goal is to infer a sensitive attribute of a secret input. Although this sensitive information may not leak the identity of the user, they still need to be protected. For instance, leaking information about users health condition or political view is sensitive.

\textbf{Re-Identification.} If the same user sends other queries at different times even if the identification of the user is hidden. This information is sensitive in the health-care applications when the same user sends multiple queries. This attack plays an important role when the attacker have access to multiple systems and can Re-Identify same user whitin multiple systems. 

\textbf{Distribution Leak.} Even if the attacker cannot find out the feature values of the users, changes in the distribution can be observed over time. In some applications, such as political applications this information is sensitive because it can indicate a shift in people's opinions.


\textbf{Membership Inference.} Given a data instance and (black-box or white-box) access to a pre-trained target model, a membership inference attack speculates whether or not the given data instance has contributed to the training step of the target model. One difference between the Machine Learning Membership attack~\cite{zhang2021membership} and this attack in recommendation systems is that the output in recommendation systems is that the adversary can only observe the ordered recommended items from a recommendation system instead of prediction results in the form of posterior probabilities.

\textbf{Model Inversion.} The model inversion attack extracts information from the training data used for learning the model. For a given class, the attacker, with either black-box or white-box access to the model, attempts to create an input that maximizes the confidence score of that class using the gradient descent algorithm.

\textbf{Model Stealing.} Trained models are considered the intellectual properties of their owners and can be considered confidential in many cases, therefore, extracting the model is considered a privacy breach. Apart from this, DNNs are shown to memorize information about their training data, therefore exposing the model parameters could lead to the exposure of training data. A model stealing attack is meant to recover the model parameters via black-box access to the target model.
\end{comment}

==> 8.Method.tex <==

\section{Defense Mechanism for Embedding Table Access Pattern Protection}
\label{sec:defense}

\subsection{PathORAM}
Oblivious RAM (ORAM) first introduced in~\cite{goldreich1996software} to avoid access pattern leakage.
\subsection{Pancake~\cite{grubbs2020pancake}}

\subsection{Implementing Pancake Controller with Path ORAM privacy in SGX}

\subsection{Frequency Aware Clustering + Pancake}





==> 9.Proof.tex <==
\section{Privacy Proof}
\label{sec:guarantee}
